AoI-minimizing Scheduling in UAV-relayed IoT Networks

Due to flexibility, autonomy and low operational cost, unmanned aerial vehicles (UAVs), as fixed aerial base stations, are increasingly being used as \textit{relays} to collect time-sensitive information (i.e., status updates) from IoT devices and deliver it to the nearby terrestrial base station (TBS), where the information gets processed. In order to ensure timely delivery of information to the TBS (from all IoT devices), optimal scheduling of time-sensitive information over two hop UAV-relayed IoT networks (i.e., IoT device to the UAV [hop 1], and UAV to the TBS [hop 2]) becomes a critical challenge. To address this, we propose scheduling policies for Age of Information (AoI) minimization in such two-hop UAV-relayed IoT networks. To this end, we present a low-complexity MAF-MAD scheduler, that employs Maximum AoI First (MAF) policy for sampling of IoT devices at UAV (hop 1) and Maximum AoI Difference (MAD) policy for updating sampled packets from UAV to the TBS (hop 2). We show that MAF-MAD is the optimal scheduler under ideal conditions, i.e., error-free channels and generate-at-will traffic generation at IoT devices. On the contrary, for realistic conditions, we propose a Deep-Q-Networks (DQN) based scheduler. Our simulation results show that DQN-based scheduler outperforms MAF-MAD scheduler and three other baseline schedulers, i.e., Maximal AoI First (MAF), Round Robin (RR) and Random, employed at both hops under general conditions when the network is small (with 10's of IoT devices). However, it does not scale well with network size whereas MAF-MAD outperforms all other schedulers under all considered scenarios for larger networks.

==> 5-DQN_unused_.tex <==
\subsection{Deep Q Network (DQN) based scheduler}
\label{dqn_policy}

The requirement to take into account the packet losses and the periodicity in packet generation, in addition to the AoI of the users, presents the motivation for a reinforcement learning (RL) based scheduler. In RL, an agent is able to take an informed decision on which actions to take after interacting with the environment as the interaction allows it to learn about the environment. A typical RL framework is %shown in Fig. \ref{fig:RL} 
where an agent takes an \textit{action} after observing the environment \textit{state}, following which it gets a \textit{reward} which is like a feedback of the quality of the action taken. 
%More details about these in the context of our setting will be given below.

% \begin{figure} [htb]
%     \vspace{-0.05 in}
%     \centering
%     \includegraphics[scale=0.35, trim={0cm 0cm 0cm 0cm},clip, angle=0]{images/RL_system.png}
%     \vspace{-0.1in}
%     \caption{Reinforcement Learning. \Vijay{Did you create this figure? If not, lets not use it.}}
%     \label{fig:RL}
%     \vspace{-0.05 in}
% \end{figure}

Deep Q Networks (DQN) are a special type of reinforcement learning (RL) algorithms that is based on using deep neural nets for q-learning. Q-learning is a model free approach to reinforcement learning that tries to learn the q-values for various state-action combinations and storing it in a q-table \cite{watkins1992q}. While q-learning is still suitable  for our environment comprising of discrete and finite state and action spaces, it is not a computationally feasible approach as the number of state and actions grow large. Therefore the need for a function approximator arises that is able to learn the the value function instead of storing the full q-table. Since neural networks are powerful function approximators, they can be used to approximate the value function and this is the idea behind DQNs. It was first presented in 2015 in DeepMind's seminal paper \cite{mnih2015human}. Since then, it has found use in a variety of applications and \cite{mao2018deep} lists some of the important works that involve using DQN in wireless networks. Next we describe the Markov Decision Formulation (MDP) of our setup in terms of state, actions and the state transitions. 


\subsubsection{State Space}
State can be defined in simple terms as the scenario encountered by the agent, where the agent is the BS in charge of the scheduling. For our system, we define the state at any time slot $t$ as 

\begin{align}
x(t) = (t, \{{AoI_{m}^{UAV}(t)}\}_{m=1}^{M}, \{{AoI_{m}^{BS}(t)}\}_{m=1}^{M})%, \{\hat{e}_{n}(t)\}_{n=1}^{N} )
\label{eqn:state_space}
\end{align}

\noindent where $t$ is the ongoing time slot. When the simulation starts at $t=1$, the values of the initial AoIs $AoI_{m}^{device} (t)$, $AoI_{m}^{UAV}$ and $AoI_{m}^{BS} (t)$ are initialized to 1.% and as $t$ increases, they change as described in Sec. \ref{sec:system}. 
%based on Eqn. \eqref{eqn:AoI_evolution_UAV} and Eqn. \eqref{eqn:AoI_evolution_BS}. 
The set of state space is denoted as $\mathcal{X}$ and the state transitions are given by Eqn. \eqref{eqn:transition_AoI_UAV_sample},  Eqn. \eqref{eqn:transition_AoI_UAV_no_sample}, Eqn. \eqref{eqn:transition_AoI_BS_update} and Eqn. \eqref{eqn:transition_AoI_BS_no_update}.
 %where $\hat{e_n}$ is the estimated of the update loss probability between UAV $n$ and BS. The BS doesn't know the quality of the update loss probability for each UAV-BS link $\hat{e}_{n}$ and hence they are initialized at $t=1$ as 1. As $t$ increases, $\hat{e}_{n}$ is updated based on the proportion of successful updates and will try to approach the correct value of $e_{n}$.
 
 

\subsubsection{Action Space}
As described in Sec. \ref{sec:system}, scheduling involves two simultaneous steps of sampling users and updating UAVs at each slot. Therefore the action at each slot $(t)$ is given as 

\begin{align}
    \alpha(t) = (\mathcal{S}(t), \mathcal{U}(t))
    \label{eqn:action_space}
\end{align}

\noindent where $\mathcal{S}(t)$ is the list of all users sampled by all the UAVs at slot $t$. $\mathcal{S}(t) = \{S_1(t), S_2(t),...S_n(t)\}$ such that $|S_n(t)| \le L$. Similarly, $\mathcal{U}(t) $ is the list of users selected to forward their stored information to the BS where $|\mathcal{U}(t)| \le K$. The set of all possible values of action is denoted as $\mathcal{A}$.


\subsubsection{Reward}
As the objective is improving the information freshness at the BS, the reward is given by the negative of the sum AoI of all the users at the BS at each time step $t$, as shown in Eqn. \eqref{eqn:reward_fn}. 

\begin{align}
    r(x(t), \alpha(t)) = r(t) = -\sum_{m=1}^{M} AoI_m^{BS}(t)
    \label{eqn:reward_fn}
\end{align}

It can be seen that the MDP can be modelled as a finite horizon MDP with finite and discrete state and action spaces. But $x$ is very high dimensional due to which the standard finite-horizon dynamic programming algorithm cannot be used \cite{abd2019deep}. As mentioned before, DQN is suitable for scenarios like this. 


% The overall objective is to learn the optimal policy that will maximize the cumulative reward given by Eqn. \eqref{eqn:cum_reward}

% \biplav{check r(t) or r(t+1), one in Eqn and one in the 2nd last line}

% \begin{equation}
%     \max_{\pi} Q(t) = \max_{\pi} \mathbb{E}[r(t)+\gamma r(t+1)+\gamma^2 r(t+2)+..|x(t),a(t), \pi]
%     \label{eqn:cum_reward}
% \end{equation}

% where $\gamma$ is the discount factor on future rewards. 

% \noindent 
In DQN, the agent interacts with the environment states through actions with the objective of maximizing the cumulative reward. Considering the environment’s current state as $x(t)$, the agent selects action $\alpha(t)$ from its action space following policy $\pi$. The environment then transitions to the new state $x(t+1)$ according to the state transition probabilities described in Eqn. \eqref{eqn:transition_AoI_UAV_sample}, \eqref{eqn:transition_AoI_UAV_no_sample}, \eqref{eqn:transition_AoI_BS_update}, \eqref{eqn:transition_AoI_BS_no_update} while resulting an award $r(t)$. The objective of using the DQN is to find the optimal policy $\pi^*$ under which the sum AoI of all devices at the BS given by Eqn. \eqref{eqn:BS_AoI_sum} is minimized. In the framework of q-learning, a state-action value function $Q^{\pi}(x(t),\alpha(t))$ is defined as the net reward when the system performs action $\alpha(t)$ while starting from state $x(t)$ and then follows policy $\pi$. Q-learning tries to calculate the q-function by learning a policy which will maximize the cumulative reward. This is done using the Bellman update rule using Eqn. \eqref{eqn:q_function} 

\begin{multline}
    Q_{t+1}(x(t),a(t))=Q_{t}(x(t),a(t)+ \\ \beta(r(t)+\gamma \min_{\alpha} Q_{t} (x(t+1),\alpha)-Q_{t}(x(t),\alpha(t)))
    \label{eqn:q_function}
\end{multline}

\noindent where $r(t)$ is the instantaneous reward at slot $t$ and is calculated using Eqn. \eqref{eqn:reward_fn}. $\beta$ and $\gamma$ are the learning rate and the discount factor respectively. Therefore the agent approximates the q-function using Eqn. \eqref{eqn:q_function} and then takes the action that maximizes the reward. As the agent will not have the correct estimate of the q-values corresponding to many state-action pairs as a consequence of not visiting them, it needs to explore in addition to exploiting the known values of state-action pairs. This is known as the exploration-exploitation trade-off. An epsilon ($\epsilon$) greedy approach where the agent takes a random action with the objective of exploring the environment with probability $\epsilon$ and acts greedily with probability $1-\epsilon$ is generally used to ensure the agent doesn't get stuck with sub-optimal actions. We use a decaying epsilon approach where the value of $\epsilon$ is gradually reduced from $\epsilon_{start}$ to $\epsilon_{end}$ using a polynomial decay function \cite{tfcompat30:online} with a step-wise decay every $d$ episodes that ensures less exploration as the learning proceeds.

While Eqn. \eqref{eqn:q_function} can be theoretically used for all scenarios, its iterative nature makes it infeasible to be used for large state spaces as it will suffer from very slow convergence in addition to needing a large memory \cite{abd2019deep}. Moreover this approach cannot be used when there are unobserved states \cite{powell2007approximate} and visiting every state-action pair is not practical. This is where the approximating power of neural networks are put to use as they can extract the important features from the available data points and summarize them in smaller dimensions. Neural networks approximates the q-function as $Q(s,\alpha|\theta)$ where $\theta$ are its weights. We use a fully connected neural network with two hidden layers $H_1 \times H_2$. The number of neurons at the input and output layers are $|\mathcal{X}|$ and $|\mathcal{A}|$ respectively. 
The weights at iteration $k+1$ are updated based on the loss calculated in iteration $i$ using Eqn. \eqref{eqn:loss} so that the q-function can be approximated as accurately as possible.  

\begin{multline}
    L(\theta_{i+1}) =  \\ (r(t)+\gamma \min_{\alpha'}Q(r(t+1),\alpha'|\theta_{i}) - Q(r(t),\alpha'|\theta_{i+1}))^2
    \label{eqn:loss}
\end{multline}

At each time step, the experience of the agent is stored in \textit{experience replay} which is also called replay memory that is set to a fixed size $R$. The experience at time $t$ is denoted as $exp(t) = (x(t),\alpha(t),r(t),x(t+1))$ and provides a summary of the agent’s experience at that time. The replay memory is then used to randomly sample a batch of stored experiences which will be used to train the neural network. The primary benefit of using random samples from replay memory to learn instead of consecutive samples as the agent encounters them is that consecutive experiences have high correlation which may lead to inefficient learning \cite{8382166}. Therefore at each episode, a batch of $B$ past experiences are fed as an input to the DQN and the gradients of the weights are calculated as shown in Eqn. \eqref{eqn:batch_gradient}.


\begin{multline}
    \nabla{\theta_{i+1}}L(\theta_{i+1}) =  \\ (r(t)+\gamma \min_{\alpha'}Q(r(t+1),\alpha'|\theta_{i}) - Q(r(t),\alpha'|\theta_{i+1})) \times \\
    \nabla{\theta_{i+1}}Q(s(t),\alpha(t)|\theta_{i+1})
    \label{eqn:batch_gradient}
\end{multline}


The DQN based scheduler is explained in Algorithm \ref{algorithm - dqn} and is shown in Fig. \ref{fig:dqn}.



\begin{algorithm}[t]
	\caption{DQN scheduler}
	\begin{algorithmic}[1]\small 
		\State Initialize a neural network along with the necessary hyper-parameters and a replay memory. Set iteration $i=1$.
		\State \textbf{Repeat:}
		\State \quad Set $t=1$ and observe initial state $ x(1) $.
		\State \quad \textbf{Repeat:}
		\State \quad \quad Select an action $ \alpha $:
		\State \quad \quad \quad select a random action $\alpha \in \mathcal{A}$ with probability $ \epsilon $ ,
		\State \quad \quad \quad otherwise select $ \alpha = \argmin_{\alpha} Q(x(t),\alpha|\boldsymbol{\theta}_k) $.
		\State \quad \quad Perform action $ \alpha $. 
		\State \quad \quad Observe the reward $ x(t) $ and the new state $ x(t+1) $.
		\State \quad \quad Store experience = $ \left\{x(t),\alpha(t),r(t),x(t+1)\right\} $ in the replay \Statex \quad \quad memory.
		\State \quad \quad $ t = t+1 $
		\State \quad \textbf{Until} $t$ is the terminal step, i.e. $t==T$:
% 		\State \quad Sample $B$ random experiences $ \left\{\hspace{-0.5mm}{x}(\eta), \hspace{-0.5mm}{\alpha}(\eta),\hspace{-0.5mm}{r}(\eta),\hspace{-0.5mm}\x(\eta+1)\hspace{-0.5mm}\right\} $
        \State \quad Sample a batch of $B$ experiences $x(t'),\alpha(t'),r(t'),x(t'+1)$
		\Statex \quad from the replay memory.
		\State \quad Calculate the \emph{target} value $ \tau $:
		\State \quad \quad If the sampled experience is for $ t'=1 $ then $ \tau={r}(t')  $,
		\State \quad \quad Otherwise $ \tau={r}(t') + \gamma \min_{\alpha'} Q({x}(t' + 1),\alpha'| \boldsymbol{\theta}_k) $.
		\State \quad Train the network $ Q $ using the gradient in \eqref{eqn:batch_gradient}.
		\State \quad $ i = i+1 $.
		\State \textbf{Until} i=I
	\end{algorithmic}
	\label{algorithm - dqn}
\end{algorithm}

\begin{figure} [htb]
    \vspace{-0.05 in}
    \centering
    \includegraphics[scale=0.28, trim={1cm 0cm 0cm 0cm},clip, angle=0]{images/dqn.png}
    \vspace{-0.1in}
    \caption{Deep Q Network}
    \label{fig:dqn}
    \vspace{-0.05 in}
\end{figure}
